Practical Privacy-Preserving Identity Verification using Third-Party Cloud Services and FHE (Role of Data Encoding in Circuit Depth Management)

National digital identity verification systems have played a critical role in the effective distribution of goods and services, particularly, in developing countries. Due to the cost involved in deploying and maintaining such systems, combined with a lack of in-house technical expertise, governments seek to outsource this service to third-party cloud service providers to the extent possible. This leads to increased concerns regarding the privacy of users' personal data. In this work, we propose a practical privacy-preserving digital identity (ID) verification protocol where the third-party cloud services process the identity data encrypted using a (single-key) Fully Homomorphic Encryption (FHE) scheme such as BFV. Though the role of a trusted entity such as government is not completely eliminated, our protocol does significantly reduces the computation load on such parties. A challenge in implementing a privacy-preserving ID verification protocol using FHE is to support various types of queries such as exact and/or fuzzy demographic and biometric matches including secure age comparisons. From a cryptographic engineering perspective, our main technical contribution is a user data encoding scheme that encodes demographic and biometric user data in only two BFV ciphertexts and yet facilitates us to outsource various types of ID verification queries to a third-party cloud. Our encoding scheme also ensures that the only computation done by the trusted entity is a query-agnostic "extended" decryption. This is in stark contrast with recent works that outsource all the non-arithmetic operations to a trusted server. We implement our protocol using the Microsoft SEAL FHE library and demonstrate its practicality.

==> relatedwork.tex <==
\section{Related Work}
Homomorphic Encryption techniques have received wide-scale adoption in the creation of practical secure outsourced computation applications. HE based techniques have been applied to achieve privacy-preserving set operations \cite{166, 170, 171, 172} and matrix operations \cite{176, 182, 184}. They have also been successful in privacy-preserving machine learning and data mining, with HE-based algorithms being developed for regression \cite{190, 191, 198} and classification \cite{204, 205, 206, 200} tasks. HE-based approaches also exist for more advanced applications, such as artificial neural networks \cite{210, 213} and secure image processing \cite{234, 236, 239}. 



Although not in the context of national ID systems, many applications have used homomorphic encryption techniques for the purposes of biometric authentication. In \cite{1}, the authors provide a framework for the secure verification of multiple biometric templates. Their approach involves the fusion of multiple biometric templates by either concatenating each template vector or processing each template individually and normalizing the individual scores. They use the Pallier cryptosystem \cite{pallier} to encrypt their templates and implement algorithms for both encrypted Euclidean distance and encrypted cosine similarity. Their scheme uses the fingercodes template and their secure algorithm for fingerprint matching performs without penalty to the error rate. Although their algorithm is fast, performing a comparison in only 0.5 ms with GPU acceleration, their use of PHE makes this scheme unsuitable for our requirements. Furthermore, this scheme requires the user’s collected biometric template to be sent to the server for verification in plain, which exposes the scheme to leakage attacks from honest-but-curious adversaries. 

In \cite{2}, they implement template quantization of the fingercodes template to achieve a low-bandwidth privacy-preserving Pallier-based scheme. However, their per-comparison time is $>4$ seconds, making this protocol too slow for our task. In \cite{3}, the scheme is created to target a similar privacy model to ours. They also parallelize the execution of their Euclidean distance algorithm to achieve faster multi-threaded performance. However, their scheme requires multiple rounds of communication between the central server and the third-party server, making it impractical for our objective of minimizing CS involvement. Furthermore, their matching method execution time with 192-bits of security and a polynomial modulus value of 8192 is $~1.2$ seconds. In the same settings, our algorithm executes in about 0.3 seconds, making it nearly four times as fast.

In \cite{4}, the authors introduce GSHADE, a protocol for the privacy-preserving computation of distance metrics such as Euclidean distance. This protocol works in the 2PC setting and uses correlated Oblivious Transfer as a primitive to exchange information between the client and server. This protocol is used in \cite{5} to develop a biometric authentication protocol. In this work, the authors develop a blinding technique to allow the fingerprint data to be obscured from the authenticator. Blinding allows their application to leverage incredibly fast distance computation from GSHADE for biometric authentication. However, the privacy-preserving login procedure needed in this protocol is stateful and required 3 rounds of communication, making it impractical for our task.

\cite{6} presents a TFHE-based privacy-preserving fingerprint authentication system. The authors implement arithmetic operations using logic gates to calculate Euclidean distance values across fingercode vectors. Their algorithms offer similar performance to ours, taking about 0.33 seconds per comparison. However, due to the use of TFHE, their ciphertext expansion ratio is extreme $(>5000)$ and the size of each ciphertext is in the order of megabytes. Since our system architecture requires all communication to be encrypted, this makes this protocol impractical for online-based authentication systems.

In addition to privacy-preserving distance computation, certain existing works also explore efficient HE-based comparison algorithms. In \cite{7}, the authors introduce a polynomial rank sort algorithm for efficiently sorting ciphertexts encrypted with the BGV \cite{BGV} scheme. Their algorithm implements SIMD operations using the same CRT-batching technique as our work. However, their algorithm has a high circuit depth $(>10)$, and their comparison operations are too slow for real-time verification purposes. In \cite{8}, the authors implement fast integer comparison algorithms for BGV and BFV schemes. This result offers state-of-the-art performance for homomorphic comparison, with their scheme taking only 11 milliseconds to compare two 64-bit integers. However, the system uses a very specific integer representation which is not generalizable to other comparison tasks. 

The task of privacy-preserving identity matching has also been tackled in existing research through various techniques. The OLYMPUS framework \cite{olympus} implements a privacy-preserving identity management framework which is complaint with the EU GDPR. The primary technical contribution of this framework is to provide surveillance protection against a malicious identity provider by distributing its role to several virtual identity providers. The project, however, has been developed primarily for password-based authentication, making their techniques inapplicable for our stateless framework.

% nzik, purdue
In \cite{nzik}, the authors present a privacy-preserving biometric identification scheme targeted toward IoT devices based on zero-knowledge proofs. Although the scheme is theoretically proven to be perfectly complete and perfectly zero-knowledge, it requires a large computation and communication overhead for each comparison, making it unsuitable for practical deployment. A similar protocol is presented in \cite{purdue} which uses non-interactive zero-knowledge and permissioned blockchains. The zero-knowledge prover in this protocol executes its proof in $>3$ in the 128-bit security setting, making it more than $10 \times$ slower that the protocol presented in this thesis.  

%BlindIM
In \cite{blindidm}, the authors present \texttt{BlindIdM}, a privacy-preserving cloud-based framework that achieves Identity Management as a Service (IDaaS). This scheme follows a similar model to ours as it involves a semi-honest third-party which can \textit{blindly} verify user identity. The scheme is based on the Security Assertion Markup Language (SAML 2.0) and requires multiple rounds of communication between the Service Provider (SP) and the cloud-based third party for identity verification.  

\cite{ppbm} presents a formal protocol for outsourced privacy-preserving biometric matching using FHE. The protocol setup in this scheme is similar to the one presented in this thesis, with the absence of a trusted central server. Furthermore, this protocol is formally proved to be \textit{IND-CPA} secure. However, the authors only create naive implementations of the comparisons, resulting in their algorithms requiring several minutes per comparison when using the TFHE encryption scheme. 
